Batch Hop-Constrained s-t Simple Path Query Processing in Large Graphs

Hop-constrained s-t simple path (HC-s-t path) enumeration is a fundamental problem in graph analysis. Existing solutions for this problem focus on optimizing the processing performance of a single query. However, in practice, it is more often that multiple HC-s-t path queries are issued simultaneously and processed as a batch. Therefore, we study the problem of batch HC-s-t path query processing in this paper and aim to compute the results of all queries concurrently and efficiently as a batch. To achieve this goal, we first propose the concept of HC-s path query which can precisely characterize the common computation among different queries.We then devise a two-phase HC-s path query detection algorithm to identify the common HC-s path queries for the given HC-s-t path queries. Based on the detected HC-s path queries, we further devise an efficient HC-s-t path enumeration algorithm in which the common computation represented by HC-s path queries are effectively shared. We conduct extensive experiments on real-world graphs and the experimental results demonstrate that our proposed algorithm is efficient and scalable regarding processing multiple HC-s-t path queries in large graphs at billion-scale.

==> index.tex <==
\section{Index Construction Optimization}
\label{sec:index}

%Based on the above analysis, we aim to devise a batch processing algorithm which can \textit{efficiently} find all \hcstps for a group of queries. The design goals of our new approach are: (1) \emph{Efficient index construction}. Our approach should construct the index for all queries efficiently by fully exploiting the computation sharing opportunities among them. The constructed index should own the same pruning ability as in \senum;  (2) \emph{Efficient path enumeration}. Our approach should significantly reduce the processing time of path enumeration by effectively identifying and sharing the common enumeration between the queries.

%Following the above idea, an overview of our algorithm is shown in \reffig{overview}. Given a graph $G$ and a set of \hcstp enumeration queries $Q$, we first efficiently build an index for all queries to reduce the number of edges involved in the subsequent enumeration. Next, we detect the common enumeration between the queries. Specifically, we propose a novel similarity function to cluster the queries such that those which are likely to share common computation are divided into the same group. The common enumeration is then extracted between query pairs within each group. Moreover, we observe that the execution order of the queries can significantly affect the memory size of cached results and the effectiveness of results utilization. Therefore, we optimizes the execution order of the queries by a greedy optimizer. Lastly, we run path enumeration on all queries as a whole following the optimized query execution order, which shares the computation and efficiently finds all \hcstps.

Hereafter, we present our multiple query optimization for \hcstp enumeration. In this section, we focus on the index construction optimization and delay the introduction on path enumeration optimization to the following sections.  

As analyzed in \refsec{exist}, \senum constructs the index for queries independently, which leads to a high index construction cost. However, the index construction procedures of different queries often have overlaps in terms of their search space. Take $q_0$ and $q_1$ in \reffig{baseline} as an example. It is clearly that  $q_0.s = v_0$ and $q_1.s=v_2$  share the same \kw{BFS} exploration starting from $v_1$ and $v_4$ during the index construction for $q_0$ and $q_1$. Apparently, if we can share these duplicate computation among different queries during the index construction, we improve the  performance of the index construction.

%these duplicated visits can be completely shared to reduce the overall cost, whereas such opportunities of computation sharing is missing in the index construction of \senum. 

% and the effective computation sharing among them can significantly reduce the overall cost. Moreover, it is analyzed in \refthm{senum} that the time complexity of index construction in \senum is $O(|Q| \cdot (|E(G)| + |V(G)|))$, where the size of $|Q|$ can be huge. 
 
 Intuitively, we can consider all queries as a whole and proceed their \kw{BFS} exploration hop by hop. In each hop, if two queries are to explore the same vertex, their individual explorations are combined and their index construction share the same procedure afterwards. Formally, let $\mathcal{T}(u, k)$ be the set of vertices visited by a \kw{BFS} from $u$ with depth $k$ and $\mathcal{V}(s, i)$ be the set of vertices $v$ with $\kw{dist}(s, v) = i$, we have: 
 
 
 %In this way, the index construction cost can be bounded by  $O(k_{max} \cdot (|E(G)| + |V(G)|))$, where $k_{max}$ is the maximum hop length among all queries and is typically much smaller than $|Q|$. Based on these intuitions, we propose \mic that \textit{efficiently} constructs the index for all queries \textit{concurrently}.


%As the size of $|Q|$ can be huge while the maximum hop constraint $k_{max}$ is significantly smaller, another question that arises is, would it be possible to reduce the cost of index construction  by dividing the construction into $k_{max}$ rounds and merging queries' computation in each round? Based on these intuitions, we propose \mic that \textit{efficiently} constructs the index for all queries \textit{concurrently}.

%to $O(k \cdot (|E(G)| + |V(G)|))$



%\begin{lemma}
%Given a query $q$, $\mathcal{T}(q.s, q.k) = \mathcal{T}(q.s, q.k-1) \cup \mathcal{V}(q.s, q.k) = \bigcup_{1 \le i \le k}{\mathcal{V}(q.s, i)}$.
%\end{lemma}

\begin{lemma}
\label{lem:index_pre}
Given a set of queries $Q$, $\cup_{q \in Q}{\mathcal{T}(q.s, q.k)} = \cup_{q \in Q}{\cup_{1 \le i \le q.k}{\mathcal{V}(q.s, i)}} \subseteq \cup_{1 \le i \le k_{max}}{\cup_{q \in Q}{\mathcal{V}(q.s, i)}}$, where $k_{max} = \max_{q \in Q}{q.k}$. 
\end{lemma}

\myproof Since a \kw{BFS} staring from $s$ with a maximum depth of $k$ can only explore the vertices $v$ with $\kw{dist}(s, v) \le k$,  we have $\cup_{q \in Q}{\mathcal{T}(q.s, q.k)} = \cup_{q \in Q}{\cup_{1 \le i \le k}{\mathcal{V}(q.s, i)}}$. Moreover, for any $q \in Q$, $q.k \le k_{max}$ and ${\cup_{1 \le i \le q.k}{\mathcal{V}(q.s, i)}} \subseteq \cup_{1 \le i \le k_{max}}{\mathcal{V}(q.s, i)}$,  thus   $\cup_{q \in Q}{\cup_{1 \le i \le q.k}{\mathcal{V}(q.s, i)}} \subseteq \cup_{1 \le i \le k_{max}}{\cup_{q \in Q}{\mathcal{V}(q.s, i)}}$. \eop


%\begin{lemma}
%Given a set of queries $Q$ and a search depth $i$, $\bigcup_{q \in Q}{\mathcal{V}(q.s, i)} \subseteq V(G)$.
%\end{lemma}

\begin{lemma}
\label{lem:index}
Given a set of queries $Q$, $\cup_{q \in Q}{\mathcal{T}(q.s, q.k)} \subseteq \cup_{1 \le i \le k_{max}}{V(G)}$.
\end{lemma}

\myproof  This lemma can be proved directly according to \reflem{index_pre}   \eop





\iffalse
\begin{lemma}
Given a hop length $k$ and two vertices $u$ and $v$. If $u.\nbrout \cap v.\nbrout \ne \emptyset$, then
\begin{center}
$\mathcal{T}(i, k) \cup \mathcal{T}(v, k)$ = $\bigcup_{i \in (u.\nbrout \backslash v.\nbrout)}{\mathcal{T}(i, k)}\ \cup$ 

$\hspace{30.6mm} \bigcup_{j \in (v.\nbrout \backslash u.\nbrout)}{\mathcal{T}(j, k)}\ \cup$

$\hspace{30.5mm} \bigcup_{w \in (u.\nbrout \cap v.\nbrout)}{\mathcal{T}(w, k)} $.
\end{center}
\end{lemma}
\fi


According to \reflem{index}, the process of index construction on individual queries can be combined and converted to a concurrent graph exploration consisting of $k_{max}$ rounds, and at most  vertices in $G$ are visited in each round.  Following this idea, our new index construction  algorithm \mic is shown in \refalg{mic}. %executes in an iterative manner with a total of $k_{max}$ rounds. In each round $i$, all queries run their breadth-first search together, where exploration on the same vertices are merged. Specifically, for every vertex $v$ in $G$, $\kw{dist}(q.s, v) = i$, or $\kw{dist}(v, q.t) = i$ if searched in the reversed direction, is stored in the index for queries $q$ that are concurrently exploring $v$ in current round.

%Given a query set $Q$ where the largest hop constraint among all queries is $k'$, the index construction finishes in $k'$ scans on the graph vertices. 



%The structure of Shortcut-Graph is a graph $G^*$ that connects the vertices from input graph $G$ with shortcuts. For each $v \in V(G)$, ... $\square$

%In a nutshell, \mic executes in an iterative manner, which takes as input the graph $G$ and a set of \hcstp queries $Q$. Each iteration $i$ contains three steps: (1) The vertices in $G^*$ are scanned in sequential order. (2) We only choose the vertices whose encountered queries need to be handled immediately, so that the query's index construction can be finished before the end of all iterations. The rest of the vertices are skipped instead. (3) For each vertex $v$  to be processed and $v' \in G.\nbrout(v)$, the new shortcuts (i.e. $G^*.\nbrin(v')$) are then updated accordingly and the queries residing on $v$ continue moving to $G.\nbrout(v)$. The index construction in the reversed direction can be achieved by running \mic on $G^r$. 

\begin{algorithm}[htb]
  \SetAlgoLined\DontPrintSemicolon
  %\textbf{Input:} Leaf Index $I$, Current Level $L$, Search Width $\Delta$,\\
  %\hspace{9mm}Cache $C$, RPC Batch Size $B$, hc-s-t Path Set $P_k$\\
  \nl $k_{max} \leftarrow \max_{q \in Q} q.k$; $I \leftarrow \emptyset$;\\
  \nl \ForEach{$q \in Q$} {
  \nl $q.s.\kw{curQ}.\kw{add}(q);$}
  \nl \ForEach{$i \in 0..k_{max}$}{
  \nl \ForEach{$v \in V(G)$}{
  \nl \If{ $ \exists ~q \in v.\kw{curQ}$ s.t. $q.k \ge k_{max} - i$}{
  \nl \ForEach{$v' \in \ \nbrout(v)$}{
  %\nl $v'.\kw{curQ}$ += $[v.\kw{curQ}\ \backslash \ v'.\kw{preQ}]$;\\
  \nl \ForEach{$q \in v.\kw{curQ}$}{
  \nl \textbf{if} $q \not\in v'.\kw{preQ}$ \textbf{then} $v'.\kw{curQ}.\kw{add}(q)$; \\
  }
  
  %\nl $v'.\kw{curQ} += \{\forall q \in v.\kw{curQ} \mid q \not\in v'.\kw{preQ}\}$\\
  \nl \ForEach{$q \in v'.\kw{curQ}$}{
  \nl \If{$q.\kw{init}$ is not initialized} {
  \nl $q.\kw{init} \leftarrow i$;
  }
  \nl $I.\kw{add}(q.s, v', i - q.\kw{init}+1)$;\\
  \nl \textbf{if} $q.t = v'$ \textbf{then} $v'.\kw{curQ}.\kw{remove}(q)$;\\
  }
  }
  \nl $v.\kw{preQ} \leftarrow v.\kw{preQ} \cup v.\kw{curQ}; v.\kw{curQ}.\kw{clear}()$;
  }
  }
  }
  \nl \textbf{return} $I$;
  
  \caption{\kwnospace{IndexConstruction}($G, Q$)}
  \label{alg:mic}
\end{algorithm} 


\stitle{Algorithm.} In \refalg{mic}, for each vertex $v \in G$, $v.\kw{curQ}$ stores the set of queries that are currently exploring $v$, and $v.\kw{preQ}$ stores the set of queries that have explored $v$ before. It first finds the largest hop constraint $k$ among all queries as $k_{max}$, which represents the maximum number of rounds required to finish the index construction for all queries. For each query $q$, \mic adds $q$ to $q.s.\kw{curQ}$ for initialization (line 2-3). Then, in each round, it scans the vertices $v \in G$,  if $v$.\kw{curQ} contains any query $q$ whose hop constraint $k$ is not less than the number of rounds left, then for each of $v$'s out-neighbors $v'$, (1) the queries $q$ from $v.\kw{curQ}$ are added to $v'$.\kw{curQ} if $q \notin v'.\kw{preQ}$ (line 8-9); (2) for each query $q$ in $v'$.\kw{curQ}, if $q$ has never been processed before, $q.\kw{init}$ is initialized as  $i$ (line 10-12). Then $\kw{dist}(q.s, v') = i-q.\kw{init}+1$ is inserted into the index $I$ (line 13). If $v' = q.t $, it means the exploration regarding $q$ is finished, and $q$ is removed from $v'.\kw{curQ}$ (line 14). After all queries in $v.\kw{curQ}$ are iterated, all queries in $v$.\kw{curQ} are moved to $v$.\kw{preQ} (line 15). The index construction is finished at $k_{max}$ round and $I$ is  returned in line 16. \refalg{mic} only shows the index construction in the forward direction, and that in the reversed direction can be directly achieved by replacing $G$ with $G^r$ and $q.s$ with $q.t$.

\iffalse
\begin{figure}[htb]
  \centering
  \includegraphics[width=0.9\columnwidth]{figures/construction.pdf}
  \vspace{-3mm}
  \caption{Example of \mic}
  \label{fig:mic}
  \vspace{-3mm}
\end{figure}
\fi


%\begin{figure}[htb]
%  \centering
%  \includegraphics[width=\columnwidth]{figures/example_index.pdf}
%  \caption{Example of \mic}
%  \label{fig:mic}
%\end{figure}
%
%\begin{table}[h!]
%\caption{\mic States}
%\centering
%\begin{tabular}{c | c | c} 
% \hline
%  Round & $v.\kw{curQ}$ & $\Delta I$  \\ 
% \hline
% \multirow{2}{*}{0} & $v_0:\{q_0\}; v_2:\{q_1\}$ & $\{v_0, v_2, v_5\} \rightarrow \{v_1\}$ \\ 
% & $v_5:\{q_2\}$ &$\{v_0, v_2\} \rightarrow \{v_4\}$ \\
% \hline
% \multirow{2}{*}{1} & {$v_1:\{q_0, q_1, q_2\}$} & $\{v_0, v_2, v_5\} \rightarrow \{v_7, v_8\}$ \\ 
%  & $v_4:\{q_0, q_1, q_3\}$ & $\{v_0, v_2, v_4\} \rightarrow \{v_9\}$ \\
% \hline
% \multirow{3}{*}{2} & \multirow{2}{*}{$(v_7, v_8):\{q_0, q_1, q_2\}$} & $\{v_0, v_2, v_5\} \rightarrow \{v_{10}\}$ \\ 
%   & \multirow{2}{*}{$v_9: \{q_0, q_1, q_3, q_4\}$} & $\{v_0, v_2, v_4, v_9\} \rightarrow $ \\
%   &&$\{v_{15}, v_8, v_3\}$\\
% \hline
%  \multirow{3}{*}{3} & $v_8:\{q_3, q_4\}$ & \multirow{2}{*}{$\{v_0, v_2, v_5\} \rightarrow \{v_{12}\}$} \\ 
%   & $v_{10}:\{q_0, q_1, q_2\}$ & \multirow{2}{*}{$\{v_0, v_2, v_4, v_9\} \rightarrow \{v_6\}$} \\
%   & $(v_3, v_{15}): \{q_0, q_1, q_3, q_4\}$ & \\
% \hline
% \multirow{2}{*}{4} & $v_{12}:\{q_0, q_1\}$ & $\{v_0, v_2, v_4, v_9\} \rightarrow$ \\ 
%   & $v_6: \{q_0, q_1, q_3, q_4\}$ & $\{v_{11}, v_{13}, v_{14}\}$ \\
%    \hline
% \multirow{2}{*}{5} & $(v_{11}, v_{13}, v_{14}):$ & \multirow{2}{*}{$\emptyset$} \\   
% & $\{q_0, q_1, q_3, q_4\}$ &\\
% \hline
%\end{tabular}
%\label{tab:index}
%\end{table}

\begin{figure}[htb]
  \centering
  \includegraphics[width=\columnwidth]{figures/example_index.pdf}
      \vspace{-5mm}
  \caption{Example of \mic}
  \label{fig:mic}
    \vspace{-5mm}

\end{figure}


\begin{example}
Reconsider $G$ and $Q$ shown in \reffig{graph}. The detailed execution of \mic is shown in \reffig{mic}, which consists of six rounds. As can be seen, a number of boxes are shown above each round $i$, which demonstrate the vertices that are visited by the concurrent breadth-first search in each round $i$. The $\kw{curQ}$ field of each vertex is also shown in the box, indicating the list of queries whose explorations are shared. 

In \textit{round} 0, as $q_0$, $q_1$ and $q_2$ all have a hop constraint $k$ of 6 that is equal to the maximum number of rounds, the search from their source vertices $S_0 = \{v_0$, $v_2$, $v_5\}$ immediately starts. Specifically, as $v_1$ and $v_4$ are found to be the common out-neighbors of $S$, the queries in the $\kw{curQ}$ field of $S_0$ are all directly moved to both $v_1.\kw{curQ}$ and $v_4.\kw{curQ}$. The shortest distance from the vertices in $S_0$ to $v_1$ and $v_4$ are subsequently added to the index, which is 1. In round 1, as $v_1.\kw{curQ}$ and $v_4.\kw{curQ}$ are both non-empty, the breadth-first search continues on them. In particular, as $v_7$ and $v_8$ are found as the out-neighbors of $v_1$, the queries $\{q_0, q_1, q_2\}$ in $v_1.\kw{curQ}$ are directly moved to $v_7.\kw{curQ}$ and $v_8.\kw{curQ}$. Similarly, as $v_9$ is the out-neighbor of $v_4$, the queries ${q_0, q_1, q_2}$ in $v_4.\kw{curQ}$ are also moved to $v_9.\kw{curQ}$. Additionally, the shortest distance from $v_1$ to $v_7$, $v_1$ to $v_8$ and $v_4$ to $v_9$ are inserted into the index, which are 2. The algorithm in the following rounds is similarly executed, where the searched vertices and their $\kw{curQ}$ field are shown in \reffig{mic}.
\end{example}

%Initially, each query $q$ is added to the \kw{curQ} field of its source vertex $s$. In \textit{round} 0, as $q_0$, $q_1$ and $q_2$ all have a hop constraint $k$ of 6 that is equal to the maximum number of rounds, their source vertices $v_0$, $v_2$ and $v_5$ are immediately processed. In contrast, $q_3$ and $q_4$ are skipped instead. As $v_1$ is found to be the common out-neighbor of these three processed vertices, edges from each of them to $v_1$ are added to $G^*$, with a weight of $i - q.\kw{init} + 1 = 1$. The three queries are also inserted into $v_1.\kw{curQ}$. Similarly, as $v_4$ is an out-neighbor of $v_0$ and $v_2$, edges from $v_0$ and $v_2$ to $v_4$ are added to $G^*$ with a weight of 1, and $q_1$ and $q_2$ are inserted into $v_4.\kw{curQ}$. At the end of \textit{round} 0, $v_0$, $v_2$ and $v_5$ migrate the processed queries from their \kw{curQ} field to \kw{preQ}. In \textit{round} 1, we perform a sequential graph scan and find that $v_1$ and $v_4$ both contain a query $q$ in their \kw{curQ} field where $q.\kw{i} + i \ge d$. As $q_3$ presents in $v_4.\kw{curQ}$, its index construction simultaneously starts. Similar to \textit{round} 0, as $v_1.\kw{curQ} = \{q_0, q_1, q_2\}$ and $v_4.\kw{curQ} = \{q_0, q_1, q_3\}$, edges of $\{v_0, v_2, v_5\} \cdot \{v_7, v_8\}$ and $\{v_0, v_2\} \cdot \{v_9\}$ are inserted into $G^*$ with a weight of $2$. Additionally, because $q_3$ has never been processed before, an edge from $v_4$ to $v_9$ with a weight of $1$ is added to $G^*$. The same procedure repeats in the following rounds, where the processed vertices and inserted edges in each round are illustrated in \reffig{mic} (a) and (b), respectively. Note that in \textit{round} 4, because $q_2.t = v_{12}$, $q_2$ is removed from $v_{12}.\kw{curQ}$. At the end of \textit{round} 6, $G^*$ contains the edges from the queries' source vertices to all reachable data vertices, where the weight of edge $(s, v)$ indicates the minimum number of required hops to perform a promising search from vertex $v$ in the reversed direction.

The correctness of \refalg{mic} can be easily obtained following \reflem{index_pre} and \reflem{index}. Moreover, we have the following theorem on the running time of \refalg{mic}.

\begin{theorem}
\label{thm:index_cost}
Given a set of queries $Q$ and a graph $G$, the time complexity of \refalg{mic} to construct the index for $Q$ is bounded by $O(k_{max} \cdot (m + n))$.
\end{theorem}


\myproof According to \reflem{index}, the index construction consists of $k_{max}$ rounds. Moreover,  each round contains a complete exploration of $G$ in the worst case, which can be bounded by $O(m + n)$. Thus, the total cost of \refalg{mic} to construct the index  is $O(k_{max} \cdot (m + n))$. \eop

Compared with \refalg{base}, the time complexity of index construction is reduced  from  $O(|Q|\cdot(m+n))$ to $O(k_{max} \cdot (m+n))$. Considering that many graphs in the real-world have the small-world properties and even the maximum value of $k_{max}$ (diameter of $G$) would be generally much smaller than $|Q|$, our index construction algorithm is more efficient than constructing the index individually shown in \refalg{base}.




